Privacy-Enhancing Fall Detection from Remote Sensor Data Using Multi-Party Computation

Motion-based fall detection systems are concerned with detecting falls from vulnerable users, which is typically performed by classifying measurements from a body-worn inertial measurement unit (IMU) using machine learning. Such systems, however, necessitate the collection of high-resolution measurements that may violate users' privacy, such as revealing their gait, activities of daily living (ADLs), and relative position using dead reckoning. In this paper, we investigate the application of multi-party computation (MPC) to IMU-based fall detection for protecting device measurement confidentiality. Our system is evaluated in a cloud-based setting that precludes parties from learning the underlying data using multiple, disparate cloud instances deployed in three geographical configurations. Using a publicly-available dataset, we demonstrate that MPC-based fall detection from IMU measurements is practical while achieving state-of-the-art error rates. In the best case, our system executes in 365.2 milliseconds, which falls well within the required time window for on-device data acquisition (750ms).

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> sections/architecture.tex <==

\subsection{Workflow}
\label{sec:workflow}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/high-level-arch.pdf}
    \caption{High-level workflow for MPC-based fall detection.}
    \label{fig:high_level}
\end{figure}

The principle stages of the proposed system architecture are illustrated in Figure \ref{fig:high_level} and described as follows:

\begin{enumerate}
    \item \emph{Data acquisition}. The collection of tri-axial IMU data on a master device, e.g. smartphone, at an appropriate sampling frequency for fall detection. This may be unimodal input, i.e. only accelerometer~\cite{liu2012fall,mauldin2018smartfall,cao2012falld,doukas2007patient,yavuz2010smartphone}; multi-modal using, for example, accelerometer and gyroscope together~\cite{santoyo2018analysis}; or aggregating measurements from multiple sensors in a body-area network~\cite{luvstrek2009fall}.
    \item \emph{Secret sharing}. Given a data sample from a given IMU modality, $\textbf{d} = \{A_x, A_y, A_z\}$, the master device splits each component into $n$ shares using SSSS. In this work, we set $n$ equal to the number of authorised communicating parties, while the reconstruction threshold is fixed at $t=3$.  In short, IMU samples are split as follows:
    \[
\textbf{D}=
  \begin{pmatrix}
    [A_x]_0 & [A_x]_1 & [A_x]_2 & \cdots & [A_x]_n \\
    [A_y]_0 & [A_y]_1 & [A_y]_2 & \cdots & [A_y]_n \\
    [A_z]_0 & [A_z]_1 & [A_z]_2 & \cdots & [A_z]_n 
  \end{pmatrix}
\]
Where the rows comprise the individual shares of a particular component, while each column represents the $i^{th}$ share of all components.

    \item \emph{Share distribution}. The master device transmits the column elements $q \in \textbf{D}_{*j}$ to each cloud service instance individually; that is, $[A_x]_0$, $[A_y]_0$ and $[A_z]_0$, is transmitted to party $P_0$, $[A_x]_1$, $[A_y]_1$ and $[A_z]_1$ to $P_1$, and so on. By sharing each sample independently, no single cloud-based party may recover the underlying IMU samples assuming the reconstruction threshold above.  In this work, we tackle the base case that the parties are operating under an honest-but-curious model, where the protocol specification is adhered to; the focus is on protecting against unauthorised disclosure of measurements from a single compromised service, as per Section \ref{sec:threat_model}.
    \item \emph{MPC-based inferencing}.  The parties use arithmetic operations upon the received shares to perform fall detection feature extraction, such as computing the vector magnitude of IMU samples, and subsequently classification using a desired method, e.g. SVM, kNN, NB, etc.
    \item \emph{Classification decision}. The resulting label, $\textbf{L} \in \{0,1\}$, is used to denote the occurrence of a fall in a binary fashion. This value may be returned to the device in order to raise an alarm or telephone an emergency contact number, or performed by the cloud service itself.
    
\end{enumerate}



\subsection{Rationale}
\todo[inline]{Disuss why cloud based approch and not locally}

Existing work has already identified several advantages for adopting a cloud-based approach for mobility-based sensing services as opposed to, for example, a local deployment whereby IMU measurements are acquired, processed, and classified aboard the device itself~\cite{doukas2011managing,fortino2014bodycloud,gravina2017cloud}.  This includes \emph{algorithm agility} for greater flexibility in changing the underlying classification algorithm on a single or small number of servers, without potential penetration issues of updating large numbers of devices in the field.

A cloud-based approach also makes fewer assumptions about devices being able to ...

A multi-party cloud-based approach...algorithm agility/can easily make updates, resilience against compromised parties (assuming non-collusion threshold).  Bad points: communication overhead with device.

Why not fully homomorphic encryption? TEE? SE?

\todo[inline]{Forensics/auditing: trusted authority with access to cloud instances can retrieve IMU data shares}
